HRP: Human Affordances for Robotic Pre-Training

In order to *generalize* to various tasks in the wild, robotic agents will need a suitable representation (i.e., vision network) that enables the robot to predict optimal actions given high dimensional vision inputs. However, learning such a representation requires an extreme amount of diverse training data, which is prohibitively expensive to collect on a real robot. How can we overcome this problem? Instead of collecting more robot data, this paper proposes using internet-scale, human videos to extract "affordances," both at the environment and agent level, and distill them into a pre-trained representation. We present a simple framework for pre-training representations on hand, object, and contact "affordance labels" that highlight relevant objects in images and how to interact with them. These affordances are automatically extracted from human video data (with the help of off-the-shelf computer vision modules) and used to fine-tune existing representations. Our approach can efficiently fine-tune *any* existing representation, and results in models with stronger downstream robotic performance across the board. We experimentally demonstrate (using 3000+ robot trials) that this affordance pre-training scheme boosts performance by a minimum of 15% on 5 real-world tasks, which consider three diverse robot morphologies (including a dexterous hand). Unlike prior works in the space, these representations improve performance across 3 different camera views. Quantitatively, we find that our approach leads to higher levels of generalization in out-of-distribution settings. For code, weights, and data check: https://hrp-robot.github.io

==> rebuttal.tex <==

 \noindent We would like to thank the reviewers for their thoughtful comments and feedback that will no doubt strengthen the paper. We're happy: that the reviewers found our, ``idea is useful as it paves a way to leverage larger datasets outside the robotics space" (\areans); that they recognized a, ``clear hypothesis ... [with] clear quantitative improvement" (\ronens); that they appreciated our, ``many robot experiments" (\rtwons); and that they complimented our, ``modular [approach that] allows for freedom in implementation." (\rthreens) We'd like to take this opportunity to further clarify some points and potential misunderstandings below.\\

\noindent \textbf{[\area \rtwons] Defining ``Actionable Representations:"} We apologize for the vague terminology here. Our claim is not that the human actions transfer directly to the robot. Rather, we define an \textit{actionable representation} as one that enables the robot to make better decisions and more precise action predictions while solving a task. In contrast, a semantic representation (e.g., CLIP~\cite{Clip}) may focus more on higher level language concepts. We find that applying \ours results in significantly \textit{more actionable representations} measured by task success rate ($10 \text{ to } 30\%$ improvement over each baseline in Fig.~\ref{fig:main}), and credit the human action label fine-tuning for this. Because of the confusion it caused, we removed this term from the paper (abstract, introduction, methods, and discussion) and made our writing more precise.\\

\noindent \textbf{[\area \rtwons] Can alternate supervision match \ours with the same data?}  This is an intriguing question that we've attempted to answer in two ways. First, our existing results showcased that data alone is not enough, since \ours significantly improves the baseline Ego4D MAE representation (see Fig.~\ref{fig:main}), despite being sourced from the same Ego4D dataset~\cite{ego4d}. Second, we've added an additional experiment that replaced \ours's losses with a semantic classification loss, and found that performance dropped substantially (see Sec.~\ref{sec:results-alternate}). Both facts point to the importance of the specific supervision provided by \ours losses. \\

\noindent \textbf{[\area \rtwo \rthreens] Reproducibility:} We have added extra details regarding the data annotation pipeline to Sec.~\ref{sec:prelims-affordances}, and described the full implementation in Appendix F. Furthermore, we added a clear illustration of the Behavior Cloning stack in Fig ~\ref{fig:policy-training} and listed all hyper-parameters for that in Appendix G.\\

\noindent \textbf{[\rtwons] Related Work for LayerNorm:}
This is a good point, thanks! We have updated Section~\ref{sec:methods} with citations of related work, especially for finetuning LayerNorm. \\

\noindent \textbf{[\areans] Boosting \ours's Motivation:} We have provided some justification for why we believe that current pre-trained visual representations \textit{underutilize} human data, and how affordances can be a useful tool for learning manipulation and deploying robots in Section~\ref{sec:methods}, and cited related works in this area, both in representation learning and manipulation. \\

\noindent \textbf{[\rone \rtwons] Sim Evals:} Please note that a recent investigations~\cite{dasari2023datasets} found that standard sim evals (e.g., MetaWorld~\cite{metaworld}, Franka Kitchen~\cite{gupta2019relay}, Robosuite~\cite{robomimic}, etc.) poorly transfer to real world robotics settings, which we ultimately care about. As a result, we focused our effort on generating high quality real world evaluations, using A/B testing and sufficient trials (roughly \textit{3000 total}) to generate small error intervals. However, we do see the value in providing some comparison numbers in sim. As a result, we present evals on  MetaWorld \cite{metaworld}, a standard simulation benchmark, in Appendix H. Note that \ours helps on these tasks, but the effect is less dramatic than in the real world. \\

\noindent \textbf{[\rtwo \rthreens] Clarifying Distractor Experiment:} Table~\ref{tab:ood} shows that when adding distractors, performance \textit{in general} drops. Specifically, for the \texttt{Ego4D} baseline, the performance drops to 15\%, while our approach has 40\% success rate. Our hypothesis is that for Ego4D, the models are especially susceptible to distractors, and HRP helps with this issue. In the case of ImageNet, where the data is more diverse, our approach provides benefits in other ways (see Fig.~\ref{fig:main}). \\

\noindent \textbf{[\ronens] Improving Introduction:} We've adjusted the introduction to more clearly outline our contributions, and define Out-of-Distribution (OOD). Thanks for the feedback! \\

\noindent \textbf{[\ronens] Improving Figures:} We've added a Fig ~\ref{fig:policy-training}, which demonstrates the Behavior Cloning process. Thank you for the suggestion! \\

\noindent \textbf{[\rone \rthreens] Clarifying Eval Metrics:} In Fig~\ref{fig:main},~\ref{fig:ablate-nln},~\ref{fig:ablate-loss} we plot the average success rate across all three tasks (15+ trials per task), along with standard error bars to show how noisy/confident the performance is. For example, if a representation scores 5/10 on stacking, 6/10 on pouring, and 3/10 on stacking the final score is $47\% \pm 9.3\%$. This same information is presented numerically in the tables. To boost clarity, we've included a discussion of the metrics we used to evaluate each task success in Sec.~\ref{sec:results}, paragraph 4 and Appendix I. \\


\noindent \textbf{[\rtwons] Clarifying Training and Testing Settings:} This is a good point! We have clarified the details of the train/test split, the number of trials, the conditions of each trial, and how different training is from testing, as well as overall evaluation and testing details in Appendix I. Additionally, we would like to point out that ~\ref{sec:expsetup} already contains the number of demonstrations that were used to train each task (i.e. 50). Appendix A contains all the details about how the demonstrations were collected and the action spaces used.\\ 

\noindent \textbf{[\ronens] Improving Video:} Thank you for these suggestions! We've added detailed examples of success/failure cases into the video and will add narration to the camera ready version. \\

\noindent \textbf{[\rtwons] Adding Diffusion Policy Experiments:} To showcase that \ours representations are not limited to a specific implementation of behavior cloning, we've added additional experiments (see Sec.~\ref{sec:results-diffusion}) using the Diffusion Policy loss / action head. Note that \ours representations still significantly boost performance in this radically different imitation learning framework! \\

\noindent \textbf{[\rthreens] Multi-Stage Tasks:} The current toasting task is in fact multi-stage (see Sec.~\ref{sec:results}; real world tasks paragraph). We have highlighted this in the task description. In addition, we present stand-alone results for the toasting task in Appendix B and C, which showcase that \ours significantly improves performance in the multi-stage task.\\

\noindent \textbf{[\rthreens] Clarifying the Baselines:} We've added additional details regarding the training/implementation of the baseline models in Sec~\ref{sec:expsetup}. \\

\noindent \textbf{[\rthreens] Explaining the Affordance Losses:} To be clear, the affordance losses are calculated using simple L2 loss terms shown in Equations \ref{eq:loss-ct}, \ref{eq:loss-hand}, and \ref{eq:loss-obj} in Sec.~\ref{sec:methods-reprs}. For clarity, we've added a more thorough discussion to Appendix E discussing the exact sweep we used to find loss coefficients $\lambda$ in Eq.~\ref{eq:loss}. \\

\noindent \textbf{[\rthreens] Data Pre-Processing:} Appendix F has documented the exact data pre-processing pipeline used before feeding images into the behavior cloning network. Please note that all code will be released upon acceptance also! \\

\noindent \textbf{[\rthreens] Understanding Contact Loss Performance:} Our suspicion is that the contact supervision was noisy compared to the hand supervision and bounding boxes. As a result, this loss was less useful on the downstream tasks. We've added a discussion of this to Sec.~\ref{sec:results-ablate}. \\

\clearpage

